Spatiotemporal Maps for Dynamic MRI Reconstruction

The partially separable functions (PSF) model is commonly adopted in dynamic MRI reconstruction, as is the underlying signal model in many reconstruction methods including the ones relying on low-rank assumptions. Even though the PSF model offers a parsimonious representation of the dynamic MRI signal in several applications, its representation capabilities tend to decrease in scenarios where voxels present different temporal/spectral characteristics at different spatial locations. In this work we account for this limitation by proposing a new model, called spatiotemporal maps (STMs), that leverages autoregressive properties of (k, t)-space. The STM model decomposes the spatiotemporal MRI signal into a sum of components, each one consisting of a product between a spatial function and a temporal function that depends on the spatial location. The proposed model can be interpreted as an extension of the PSF model whose temporal functions are independent of the spatial location. We show that spatiotemporal maps can be efficiently computed from autocalibration data by using advanced signal processing and randomized linear algebra techniques, enabling STMs to be used as part of many reconstruction frameworks for accelerated dynamic MRI. As proof-of-concept illustrations, we show that STMs can be used to reconstruct both 2D single-channel animal gastrointestinal MRI data and 3D multichannel human functional MRI data.

==> def,eps.tex <==
% def,eps.tex
% Latex2e macros for including Encapsulated Postscript (.eps)
% /opt/gnu/tex/doc/user/grfguide.ps
% Needs: \usepackage[dvips,draft]{graphicx}
% Picture: \ineps{dir}{file}{size}
% Centered picture: \inceps{dir}{file}{size}
% Captioned figure: \figeps[htbp]{dir}{file}{size}{caption}
% Centered lr picture: \incepslr{dir}{file1}{file2}{size}
% Captioned lr figure: \figepslr[htbp]{dir}{file1}{file2}{size}{caption}
% Centered quad figure:
%	\figepsquad{size}{dir}{file1}{file2}{file3}{file4}{caption}
% "file" does not include the .eps, and also becomes the figure label.
% "size" is typically Esize.  optional argument specifies position
% note: the graphicx package has a command that can specify order of
% suffixes to try: \DeclareGraphicsExtensions{.eps,.pdf}
%
\ifx \ecaption \undefined
	\newcommand{\ecaption}{\caption}
\fi

%
% \inps{width=}{size}{dir}{root}{suffix}
%
\providecommand{\figcent}[1]		{\mbox{}\hfill#1\hfill\mbox{}}
%\providecommand{\figsuffix}		{.eps}
\providecommand{\figsuffix}		{}
\providecommand{\figsuffixc}		{.epsc}
\providecommand{\inps}[5]		{\includegraphics[#1#2]{#3/#4#5}}
\providecommand{\ineps}[4][width=]	{\inps{#1}{#4}{#2}{#3}{\figsuffix}}
\providecommand{\inepsc}[4][width=]	{\inps{#1}{#4}{#2}{#3}{\figsuffixc}}
\providecommand{\inceps}[4][width=]	{\figcent{\ineps[#1]{#2}{#3}{#4}}}
\providecommand{\inpdf}[4][width=]	{\inps{#1}{#4}{#2}{#3}{.pdf}}
\providecommand{\injpg}[4][width=]	{\inps{#1}{#4}{#2}{#3}{.jpg}}
\providecommand{\intga}[4][width=]	{\inps{#1}{#4}{#2}{#3}{.tga}}
\providecommand{\flabel}[1]		{\label{#1}} % figure label

% captioned/labeled eps, for use within a multiple-plot floating figure
\providecommand{\capeps}[4]{% dir file width caption
\inceps{#1}{#2}{#3}%
\ecaption{#4}%
\flabel{#2}}

\providecommand{\figeps}[5][htbp]{%
\begin{figure}[#1]%
\capeps{#2}{#3}{#4}{#5}%
\end{figure}}

\providecommand{\figepsc}[5][htbp]{%
\begin{figure}[#1]%
\figcent{\inepsc{#2}{#3}{#4}}%
\ecaption{#5}%
\flabel{#3}%
\end{figure}}

\providecommand{\figepsstar}[5][htbp]{%
\begin{figure*}[#1]%
\inceps{#2}{#3}{#4}%
\ecaption{#5}%
\flabel{#3}%
\end{figure*}}

%
% for 2 side-by-side
%

%
% Centered lr picture: \incepslr{dir}{file1}{file2}{size}
\providecommand{\incepslr}[4]{%
\lfill\ineps{#1}{#2}{#4}\hfill\ineps{#1}{#3}{#4}\rfill}

%
% Captioned lr figure: \figepslr[htbp]{dir}{file1}{file2}{size}{caption}
%
\providecommand{\figepslr}[6][htbp]{%
\begin{figure}[#1]%
\incepslr{#2}{#3}{#4}{#5}%
\ecaption{#6}%
\flabel{#3}%
\flabel{#4}%
\end{figure}}

%
% captioned 4 as 2by2
%

%
% Captioned quad figure:
% \figepsquad[htbp]{size}{dir}{file1}{file2}{file3}{file4}{caption}
\providecommand{\figepsquad}[8][htbp]{%
\begin{figure}[#1]%
\incepslr{#3}{#4}{#5}{#2}%
\\%
\incepslr{#3}{#6}{#7}{#2}%
\ecaption{#8}%
\flabel{#4}\flabel{#5}\flabel{#6}\flabel{#7}%
\end{figure}}


==> def,gen.tex <==
% def,gen.tex
% Latex2e general macros
% Jeff Fessler

% sections
%\providecommand{\dirtex}		{/n/ir7/y/fessler/tex}
%\providecommand{\dirtex}		{.} % use TEXINPUTS instead
\providecommand{\inputtex}[1]		{\label{#1}\input{#1}}
\providecommand{\isection}[2]		{\section{#1}\inputtex{#2}}
\providecommand{\isubsection}[2]	{\subsection{#1}\inputtex{#2}}

% latin
%\providecommand{\etal}		{\emph{et al\@.}\xspace}
\providecommand{\etal}		{et al\@.\xspace}
\providecommand{\ie}		{\emph{i.e\@.}\xspace}
\providecommand{\eg}		{\emph{e.g\@.}\xspace}
\providecommand{\cf}		{\emph{cf\@.}\xspace}
\providecommand{\defacto}	{\emph{de facto}\xspace}
\providecommand{\adhoc}		{\emph{ad hoc}\xspace}
\providecommand{\apriori}	{\emph{a priori}\xspace}

% web
%\providecommand{\myurl}[1][]	{\texttt{http://web.eecs.umich.edu/$\sim$fessler#1}\xspace}
\providecommand{\myurlold}[1][]	{\texttt{web.eecs.umich.edu/$\sim$fessler#1}\xspace}
\providecommand{\myurl}[1][]	{\url{http://web.eecs.umich.edu/~fessler#1}\xspace}
\providecommand{\myweb}		{\url{http://web.eecs.umich.edu/~fessler}\xspace}
\providecommand{\onweb}[1]	{Available from \myweb.}


% comments environments
% when using \usepackage{verbatim},
% the following allows this: \begin{comments} ... \end{comments} 
\let\comments=\comment
\let\endcomments=\endcomment

% huge comments.
% unfortunately this bashes the \begin{comment} environment in verbatim.sty
% which is why i have defined the preceding \comments environment.
\long\def\comment#1{}
\providecommand{\uncomment}[1]	{#1}


% common environments
\providecommand{\bcent}		{\begin{center}}
\providecommand{\ecent}		{\end{center}}
\providecommand{\benum}		{\begin{enumerate}}
\providecommand{\eenum}		{\end{enumerate}}
\providecommand{\bitem}		{\begin{itemize}}
\providecommand{\eitem}		{\end{itemize}}
\providecommand{\bvers}		{\begin{verse}}
\providecommand{\evers}		{\end{verse}}
\providecommand{\btab}		{\begin{tabbing}}	% use \= and \>
\providecommand{\etab}		{\end{tabbing}}
%\providecommand{\bverb}	{\begin{verbatim}}
%\providecommand{\everb}	{\end{verbatim}}

% positioning
\providecommand{\lfill}		{\mbox{}\hfill}
\providecommand{\rfill}		{\hfill\mbox{}}
\newcommand{\cent}[1]		{\lfill{#1}\rfill}
\newcommand{\adjustfullwidth}[1] {\adjustbox{width=\linewidth}{#1}}

% box with text stacked up in it
%\newcommand{\stacktext}[2][c]	{\begin{tabular}{#1}#2\end{tabular}}
\DeclareRobustCommand{\stacktext}[2][c]	{\begin{tabular}{#1}#2\end{tabular}}
\newcommand{\fsbox}[2][c]	{\fbox{\stacktext[#1]{#2}}}

\providecommand{\ul}[1]		{\underline{#1}}
\providecommand{\ebox}[1]	{\mbox{\fbox{$\displaystyle#1$}}}
\providecommand{\cbox}[1]	{\[\ebox{#1}\]}

\providecommand{\makeboxc}[2] {\makebox[#1\linewidth][c]{#2}}

% top-aligned side-by-side mini-pages
\newcommand{\minipaget}[2] {% width1 box1
\begin{minipage}[t]{#1\linewidth}\vspace*{0pt}#2\end{minipage}}
\newcommand{\minipagett}[4] {% width1 width2 box1 box2
\minipaget{#1}{#3}\hfill\minipaget{#2}{#4}}
\newcommand{\minipagettt}[6] {% width1 width2 width3 box1 box2 box3
\minipaget{#1}{#4}\hfill\minipaget{#2}{#5}\hfill\minipaget{#3}{#6}}

% bullet list with normal spacing
\newcounter{blist}
\providecommand{\blistmark}	{\makebox[0pt]{$\bullet$}}
\providecommand{\blistitemsep}	{0pt}
\providecommand{\blist}[1][]	{%
\begin{list}{\blistmark}{%
\usecounter{blist}%
\setlength{\itemsep}{\blistitemsep}%
\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}%
\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{1.2em}%
\setlength{\labelsep}{0.5\leftmargin}% centers label in margin
\setlength{\labelwidth}{0em}%
#1}% user over-rides
}
\providecommand{\elist}		{\end{list}}
\providecommand{\elistup}	{\elist\vspace{-\parskip}} % no space after

% enum list with normal spacing
%\providecommand{\bcolor}[1] {#1}
\providecommand{\blistitemsep}	{0pt}
\providecommand{\bjfenum}[1][]	{%
\begin{list}{\bcolor{\arabic{blist}.} }{%
\usecounter{blist}%
\setlength{\itemsep}{\blistitemsep}%
\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}%
\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{0.0em}%
\setlength{\labelsep}{1.0\leftmargin}% label in margin?
\setlength{\labelwidth}{0pt}%
#1}% user over-rides
}

% Alpha list with normal spacing
\newcounter{blistAlph}
\providecommand{\blistAlph}[1][]
{\begin{list}{\makebox[0pt][l]{\Alph{blistAlph}.}}{%
\usecounter{blistAlph}%
\setlength{\itemsep}{0pt}\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{1.2em}%
\setlength{\labelsep}{1.0\leftmargin}% letter at left side of margin
\setlength{\labelwidth}{0.0\leftmargin}#1}%
}

% Roman list with a bit of spacing
\newcounter{blistRoman}
\providecommand{\blistRoman}[1][]
{\begin{list}{\Roman{blistRoman}.}{%
\usecounter{blistRoman}%
\setlength{\itemsep}{0.5em}\setlength{\parsep}{0pt}%
\setlength{\parskip}{0pt}\setlength{\partopsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{4em}%
\setlength{\labelsep}{0.4\leftmargin}
\setlength{\labelwidth}{0.6\leftmargin}#1}%
}

%
% Portrait
% use \pagesize[.2in]{5in}{7in} to center width and height
% first argument is optional parindent
% at top of page: 1in, \topmargin, \headheight(for header), \headsep
%
\providecommand{\myheadheight}	{0in}
\providecommand{\myheadsep}	{0in}
\providecommand{\Halfheight}	{5.5in}		% half of 11" vertical page
\providecommand{\Halfwidth}	{4.25in}	% half of 8.5" horizontal page
\providecommand{\pagesize}[3][\parindent]{
\setlength{\parindent}{#1}
\setlength{\textwidth}{#2}
\setlength{\textheight}{#3}
\setlength{\headsep}{\myheadsep}
\setlength{\headheight}{\myheadheight}
\setlength{\oddsidemargin}{\Halfwidth}
\addtolength{\oddsidemargin}{-0.5\textwidth}
\addtolength{\oddsidemargin}{-1in}
\setlength{\evensidemargin}{\oddsidemargin}
\setlength{\topmargin}{\Halfheight}
\addtolength{\topmargin}{-0.5\textheight}
\addtolength{\topmargin}{-0.5\headheight}
\addtolength{\topmargin}{-0.5\headsep}
\addtolength{\topmargin}{-1in}
}

%
% Landscape
% use \pagesizeland[.2in]{5in}{7in} to center width and height
% first argument is optional parindent
%
\providecommand{\pagesizeland}[3][\parindent]{
\setlength{\parindent}{#1}
\setlength{\textwidth}{#2}
\setlength{\textheight}{#3}
\setlength{\headsep}{0.0in}
\setlength{\headheight}{0.0in}
\setlength{\oddsidemargin}{5.5in}
\addtolength{\oddsidemargin}{-0.5\textwidth}
\addtolength{\oddsidemargin}{-1in}
\setlength{\evensidemargin}{\oddsidemargin}
\setlength{\topmargin}{4.25in}
\addtolength{\topmargin}{-0.5\textheight}
\addtolength{\topmargin}{-1in}
}

%
% half of top margin for headings.
%
\providecommand{\pagehead}{%
\setlength{\headsep}{\topmargin}%
\addtolength{\headsep}{1in}%
\setlength{\headsep}{0.5\headsep}%
\setlength{\headheight}{\headsep}%
\setlength{\topmargin}{-1in}%
}


==> def,math.tex <==
% def,math.tex
% latex2e definitions of math symbols

% todo: to fix fonts see http://tug.org/fonts/fontinstall.html
%\usepackage{bbm} % black-board math
%\providecommand{\jfbbm}[1]	{\xmath{\mathbbm{#1}}} % needs bbm package
%\providecommand{\jfbbm}[1]	{\xmath{\mathsf{#1}}} % todo: while bbm broken
\providecommand{\jfbbm}[1]	{\xmath{\mathbb{#1}}}

\providecommand{\qed}[1][0pt]	{\hfill\raisebox{#1}{\inmath{\Box}}} % need latexsym package
% the next command is my favorite way to define bold letters.
% it requires \usepackage{bm,jf-fun}
\providecommand{\blmath}[1]	{\jfunl{\bm{#1}}}	% bm, jf-fun

% symbols that might need defined in a symbol table
\providecommand{\bigone}[1][\Large]	{\mbox{ {#1 1}}\xspace}
%\providecommand{\indic}[2][\large]	{\xmath{\mbox{{#1 $1$}}_{\braces{#2}}}}
% another option for \indic would be \iota (or \rchi in jf-all.sty)
\providecommand{\indic}[2][]	{\xmath{\jfbbm{I}_{\braces{#2}}}}

%\providecommand{\reals}	{\xmath{\mathrm{I\kern-.2em R}}}
\providecommand{\reals}		{\jfbbm{R}}

\providecommand{\thus}		{\xmath{\stackrel{\textstyle .}{..}}}
\providecommand{\suchthat}	{\textnormal{ s.t. }}
\providecommand{\defequ}	{\stackrel{\bigtriangleup}{=}}
\providecommand{\iid}		{\stackrel{iid}{\sim}}
\providecommand{\icomplex}	{\xmath{\imath}}

\providecommand{\norm}[1]	{\xmath{\left\| #1 \right\|}}
\providecommand{\normr}[1]	{\xmath{\| #1 \|}}
\providecommand{\normb}[1]	{\xmath{\Big\| #1 \Big\|}}
\providecommand{\normbb}[1]	{\xmath{\Bigg\| #1 \Bigg\|}}
\providecommand{\floor}[1]	{\xmath{\left\lfloor #1 \right\rfloor}}
\providecommand{\ceil}[1]	{\xmath{\left\lceil #1 \right\rceil}}
%\providecommand{\inprod}[2]	{\xmath{\langle #1,\, #2 \rangle}}
\providecommand{\inprod}[2]	{\xmath{\mathop{\langle #1,\, #2 \rangle}\nolimits}}
\providecommand{\Inprod}[2]	{\xmath{\left\langle #1,\ #2 \right\rangle}}
\providecommand{\musec}		{\xmath{\mu\mathrm{sec}}}

% \modo: ordinary modulo with a bit of space: "x mod y"
\providecommand{\modo}[2]	{\xmath{#1 \mathop{\mathrm{mod}}\nolimits #2}}
% \modp: modulo with the first part in paren: "(x) mod y"
\providecommand{\modp}[2]	{\modo{(#1)}{#2}}
% \pmod: defined in amsmath to do (x mod y)


\let\equivsave\equiv
\def\equiv{\xmath{\equivsave}}

% notes
% amsmath has subscript stacking: \sum_{\substack{ n=1 \\ n \neq m}}^N
% dvips -Ppdf for making pdf files?  \special for pdf hyperlinks?

\providecommand{\sumstack}[2]	{\sum_{\substack{#1 \\ #2}}}
\providecommand{\sumno}	{\sum\nolimits}

\providecommand{\ba}[1]		{\left[ \begin{array}{#1}}
\providecommand{\ea}		{\end{array} \right]}
\providecommand{\be}		{\begin{equation}}
\providecommand{\ee}[1]		{\label{#1}\end{equation}}
\providecommand{\den}[2]	{\begin{equation} #1 \label{#2} \end{equation}}
\providecommand{\bea}		{\begin{eqnarray}}
\providecommand{\eea}[1]	{\label{#1}\end{eqnarray}}
\providecommand{\beas}		{\begin{eqnarray*}} % obsolete! use desa{}
\providecommand{\eeas}		{\end{eqnarray*}} % obsolete!
%\providecommand{\bels}		{\begin{align*}} % requires amsmath
%\providecommand{\eels}		{\end{align*}}
%\providecommand{\bels}		{\begin{align*}} % requires amsmath
\providecommand{\beals}[1][1]	{\begin{alignat*}{#1}} % requires amsmath
\providecommand{\eeals}		{\end{alignat*}}

% displayed but un-numbered (*'d) equations using aligned
\providecommand{\desa}[1]	{\begin{align*} #1 \end{align*}} % amsmath
%\providecommand{\desa}[1]	{\begin{equation*}% % (pre 2022-11-20)
%	\begin{aligned}#1\end{aligned}\end{equation*}} % amsmath
% variant where first line is moved left using \MoveEqLeft from mathtools
\providecommand{\desal}[1]	{\begin{equation*}%
	\begin{aligned}\MoveEqLeft#1\end{aligned}\end{equation*}} % amsmath

% numbered versions (these number every line unless \nonum or \notag used)
\providecommand{\dena}[2]
	{\begin{align}#1\label{#2}\end{align}} % amsmath
\providecommand{\denal}[2]
	{\begin{align}\MoveEqLeft#1\label{#2}\end{align}} % amsmath

\providecommand{\denalt}[3]{ % text eqn label
\begin{flalign}
\text{#1} && #2 &&
\label{#3}
\end{flalign}
}

% obsolete: use desa and dena instead
\providecommand{\bals}		{\begin{equation*}\begin{aligned}} % amsmath
\providecommand{\eals}		{\end{aligned}\end{equation*}}
\providecommand{\beal}		{\begin{equation}\begin{aligned}[b]}
\providecommand{\eeal}[1]	{\end{aligned}\label{#1}\end{equation}}

% these do not work:
% http://tex.stackexchange.com/questions/3169/making-a-new-environment-combining-equation-and-split/3205#3205
%\providecommand{\bal}		{\begin{align}} % amsmath
%\providecommand{\eal}[1]	{\label{#1}\end{align}}
% but this works:
\providecommand{\bale}[2]	{\begin{align}#1\label{#2}\end{align}} % amsmath


% note: \ber and \eer and \bear are all dangerous it seems.
% use \berr and bearr instead!

%\providecommand{\ber}[1]	{\bgroup\renewcommand{\theequation}{#1}\be}
%\providecommand{\eer}[1]	{\label{#1}\end{equation}\egroup}
\providecommand{\berr}[2]{
\bgroup
\renewcommand{\theequation}{#1}
\be
#2
\ee{e,#1}
\egroup
\ignorespaces
}

%\providecommand{\bear}[1]	{\renewcommand{\theequation}{#1}\bea}
\providecommand{\bearr}[2]{
\bgroup
\renewcommand{\theequation}{#1}
\bea
#2
\eea{e,#1}
\egroup
\ignorespaces
}

% can this be done?
%\providecommand{\bebox}[1][\mbox{\fbox{$\displaystyle]	{\begin{equation}#1}
%\providecommand{\eebox}[1]	{$\}\}\label{#1}\end{equation}}
%\providecommand{\eebox}[2][$\}\}]	{#1\label{#2}\end{equation}}

\providecommand{\inmath}	{\ensuremath}
\providecommand{\xmath}[1]	{\inmath{#1}\xspace}
\providecommand{\bmath}[1]	{\xmath{\bm{#1}}}	% needs \usepackage{bm}
\providecommand{\eref}[1]	{(\protect\ref{#1})}
\providecommand{\fref}[2][]	{Fig.~\protect\ref{#2}#1}
\providecommand{\conj}		{\inmath{^*}}
%\providecommand{\conj}		{\inmath{^{\star}}}
\providecommand{\conjb}[1]	{\xmath{\brak{#1}\conj}} % [ ... ]^*
\providecommand{\degr}		{\xmath{^{\circ}}}
\providecommand{\isotop}[2]	{\inmath{^{#2}}#1\xspace}

\providecommand{\conv}		{\inmath{\ast}}
\providecommand{\cconv}		{\inmath{\ast\mbox{$\!\!$}\ast}}
\providecommand{\cconvsub}	{\inmath{\ast\mbox{$\!$}\ast}}
\providecommand{\ccconv}	{\inmath{\mathbin{\ast \mbox{$\!\!$} \ast \mbox{$\!\!$}\ast}}}

\providecommand{\inv}		{\inmath{^{-\!1}}}
\providecommand{\invT}		{\inmath{^{-\!\mathrm{T}}}}
\providecommand{\invH}		{\inmath{^{-\!\mathrm{H}}}}
\providecommand{\powten}[1]	{\inmath{\cdot10^{#1}}}
\providecommand{\uminus}	{\mathord{-}}

% invisible rule to make brackets etc. bigger
\providecommand{\irule}[1][-0.7em] {\rule[#1]{0pt}{0pt}}

\providecommand{\evalat}[2]	{\left. #1 \right|_{#2}}
\providecommand{\Evalat}[3][0.7em]
	{\left. #2 \irule[-#1] \right|_{#3}}	% -0.4\baselineskip
\providecommand{\choos}[3][-0.2]
% {\xmath{\fbox{\xmath{\begin{array}{c} #2\\[#1em]#3 \end{array}}}}}
 {\xmath{\left(\begin{array}{c} #2\\[#1em]#3 \end{array}\right)}}
%\providecommand{\choos}[2]	{\xmath{\left(\stackrel{#1}{#2}\right)}}

% \parin is "mathinner" parentheses; leaves more space around nearby operations
\providecommand{\parin}[1]	{\xmath{\mathinner{\left(#1\right)}}}
\providecommand{\paren}[1]	{\xmath{\left(#1\right)}}
\providecommand{\parenb}[1]	{\xmath{\Big(#1\Big)}}
\providecommand{\parens}[1]	{\xmath{(#1)}}
%\providecommand{\of}[1]	{\!\left(#1\right)}
\providecommand{\of}[1]		{\mleft(#1\mright)}
\providecommand{\ofb}[1]	{\!\Big(#1\Big)}
\providecommand{\brak}[1]	{\xmath{\left[#1\right]}}
\providecommand{\brakleft}[1]	{\xmath{\left[#1\right.}}
\providecommand{\brakright}[1]	{\xmath{\left.#1\right]}}
\providecommand{\brakb}[1]	{\xmath{\Big[#1\Big]}}
\providecommand{\brakbb}[1]	{\xmath{\Bigg[#1\Bigg]}}
\providecommand{\braces}[1]	{\xmath{\left\{#1\right\}}}
\providecommand{\bracesb}[1]	{\xmath{\Big\{#1\Big\}}}
\providecommand{\bracesbb}[1]	{\xmath{\Bigg\{#1\Bigg\}}}
\providecommand{\abs}[1]	{\xmath{\left| #1 \right|}}
\providecommand{\absr}[1]	{\xmath{| #1 |}} % regular size
\providecommand{\absb}[1]	{\xmath{\Big| #1 \Big|}}
\providecommand{\absbb}[1]	{\xmath{\Bigg| #1 \Bigg|}}

\providecommand{\overtext}[2]	{\overbrace{#1}^{\mbox{#2}}}
%\providecommand{\undertext}[2]	{\underbrace{#1}_{\mbox{#2}}}
\DeclareRobustCommand{\undertext}[2] {\underbrace{#1}_{\mbox{#2}}}
%\providecommand{\understack}[2] {\undertext{#1}{\stacktext{#2}}}
\DeclareRobustCommand{\understack}[2] {\undertext{#1}{\stacktext{#2}}}

\providecommand{\dddot}[1]	{\inmath{#1^{(3)}}}
\providecommand{\ddddot}[1]	{\inmath{#1^{(4)}}}
\providecommand{\dsqrt}[1]	{\xmath{\sqrt{\displaystyle #1}}}

\providecommand{\xfrac}[2]	{\xmath{\frac{#1}{#2}}}
\providecommand{\Half}[1][1]	{\xfrac{#1}{2}}
\providecommand{\half}[1][1]	{\xmath{{\scriptstyle \frac{#1}{2}}}}
\providecommand{\Frac}[2]	{\xmath{{#1}/{#2}}}
\providecommand{\pfrac}[3][]	{\xmath{\!\paren{#1\frac{#2}{#3}}}}
\providecommand{\pFrac}[3][]	{\xmath{\!\paren{#1\Frac{#2}{#3}}}}
\providecommand{\dpfrac}[3][]	{\xmath{\!\paren{#1\dfrac{#2}{#3}}}}
%\providecommand{\dfrac}[2]	% conflicts with amstex
\def\dfrac#1#2{\xmath{\displaystyle\frac{#1}{#2}}}
\def\implies	{\xmath{\Longrightarrow}} % ams?

%\providecommand{\eexp}		{\xmath{\mathop{\mathrm{e}}\nolimits}}
\providecommand{\eexp}		{\xmath{\mathinner{\mathrm{e}}}}
\providecommand{\Expi}[1]	{\xmath{\eexp^{\icomplex #1}}}
\providecommand{\expi}[1]	{\xmath{\exp\of{\icomplex #1}}}
\providecommand{\Expni}[1]	{\xmath{\eexp^{-\icomplex #1}}}
\providecommand{\expni}[1]	{\xmath{\exp\of{-\icomplex #1}}}
\providecommand{\Expo}[1]	{\xmath{\eexp^{#1}}}
\providecommand{\expo}[1]	{\xmath{\exp\of{#1}}}
\providecommand{\Expn}[1]	{\xmath{\eexp^{-#1}}}
\providecommand{\expn}[1]	{\xmath{\exp\of{-#1}}}
\providecommand{\Exp}		{\expo}	% backward compat
\providecommand{\Cos}[1]	{\xmath{\cos\of{#1}}}
\providecommand{\Sin}[1]	{\xmath{\sin\of{#1}}}

%
% the following are all obsolete due to jf-fun.sty
%
\providecommand{\Normal}[1]	{{\mathcal N}\of{#1}}
\providecommand{\mathword}[3][]	{\,\inmath{\mathrm{#2}#1\of{#3}}}
\providecommand{\wordbrace}[3][]{\,\inmath{\mathrm{#2}#1\!\braces{#3}}}
\providecommand{\Poisson}[1]	{\wordbrace{Poisson}{#1}}
\providecommand{\diag}[1]	{\wordbrace{Diag}{#1}}
\providecommand{\var}[1]	{\wordbrace{Var}{#1}}
\providecommand{\cov}[1]	{\wordbrace{Cov}{#1}}
%\providecommand{\sinc}[2][]	{\mathword[#1]{sinc}{#2}}
\providecommand{\sinc}		{\Ofun{\mathrm{sinc}}}
\providecommand{\rect}[1] 	{\mathword{rect}{#1}}
\providecommand{\sgn}[1] 	{\mathword{sgn}{#1}}
\providecommand{\real}[1]	{\mathword{real}{#1}}
\providecommand{\imag}[1]	{\mathword{imag}{#1}}

\providecommand{\mystack}[2][c]	{\xmath{\begin{array}{#1} #2 \end{array}}}
\providecommand{\myvect}[2][c]	{\xmath{\brak{\mystack[#1]{#2}}}}
\providecommand{\mymat}[1]	{\xmath{\begin{bmatrix} #1 \end{bmatrix}}} % amsmath, up to 10 cols, does not require [ccc]
\DeclareRobustCommand{\pmymat}[1] {\xmath{\begin{bmatrix} #1 \end{bmatrix}}}
\providecommand{\mymatsmall}[1]	{\xmath{\left[\begin{smallmatrix} #1 \end{smallmatrix}\right]}} % amsmath, up to 10 cols, does not require [ccc]
\providecommand{\mymato}[2][]	{\xmath{\begin{bmatrix}[#1] #2 \end{bmatrix}}}
\providecommand{\leftbrace}[2][ll]	{\left\{ \mystack[#1]{#2} \right.}
\providecommand{\zeroother}	{\\ 0, & \mathrm{otherwise}}

% integrals and derivatives
\providecommand{\negint}	{-\!\!\int\!}
\providecommand{\intinf}	{\int_{\!-\infty}^{\infty}}
\providecommand{\iintinf}	{\intinf\intinf}
\providecommand{\iint}		{\int\!\!\!\int}
\providecommand{\iiint}		{\int\!\!\!\int\!\!\!\int}
\providecommand{\iiiint}	{\int\!\!\!\int\!\!\!\int\!\!\!\int}
% caution: \der \xj_n must be \der{\xj_n} to work properly!
\providecommand{\der}[1]	{\xmath{\mathop{\mathrm{d}#1}\nolimits}}
%\providecommand{\der}		{\xmath{\mathop{\mathrm{d}}\nolimits}}
%\providecommand{\der}		{\xmath{\mathrm{d}}}
\providecommand{\dxy}		{\der{x}\der{y}}
\providecommand{\dxyz}		{\der{x}\der{y}\der{z}}

\providecommand{\ddt}[1][t]	{\xfrac{\der{}}{\der{#1}}}
\providecommand{\dder}[2]	{\xfrac{\der{}^{#2}}{\der{#1}^{#2}}}
\providecommand{\fpart}[2][]	{\xfrac{\partial #1}{\partial #2}}
\providecommand{\ffpart}[2][]	{\xfrac{\partial^2 #1}{\partial #2^2}}
\providecommand{\fffpart}[2][]	{\xfrac{\partial^3 #1}{\partial #2^3}}
\providecommand{\ffpartt}[2]	{\xfrac{\partial^2}{\partial #1 \; \partial #2}}
%\providecommand{\Part}[1]	{\frac{\partial}{\partial #1}}
%\providecommand{\Partt}[1]	{\frac{\partial^2}{\partial #1}}
%\providecommand{\Parttt}[1]	{\frac{\partial^3}{\partial #1}}

\providecommand{\Gam}		{\jfunl{\Gamma}}
\providecommand{\eps}		{\jfunl{\epsilon}}
\providecommand{\veps}		{\jfunl{\varepsilon}}


% https://tex.stackexchange.com/questions/451786/how-do-i-put-a-circle-around-a-symbol
% ostar for circular convolution
\makeatletter
\newcommand{\ostar}{\mathbin{\mathpalette\make@circled\star}}
\newcommand{\make@circled}[2]{%
 \ooalign{$\m@th#1\smallbigcirc{#1}$\cr\hidewidth$\m@th#1#2$\hidewidth\cr}%
}
\newcommand{\smallbigcirc}[1]{%
 \vcenter{\hbox{\scalebox{0.77778}{$\m@th#1\bigcirc$}}}%
}
\makeatother

